Shortened Polarization Kernels

A shortening method for large polarization kernels is presented, which results in shortened kernels with the highest error exponent if applied to kernels of size up to 32. It uses lower and upper bounds on partial distances for quick elimination of unsuitable shortening patterns. The proposed algorithm is applied to some kernels of sizes 16 and 32 to obtain shortened kernels of sizes from 9 to 31. These kernels are used in mixed-kernel polar codes of various lengths. Numerical results demonstrate the advantage of polar codes with shortened large kernels compared with shortened and punctured Arikan polar codes, and polar codes with small kernels.

==> shortwindproc.tex <==
\section{Window processing of shortened polarization kernels}
%In this section we describe a window processing algorithm for shortened kernels.

\subsection{Description of window processing algorithm}
In this section we provide a brief description of window processing (WP) algorithm. This algorithm calculates $\phi$-th bit subchannel LLR 
$\bS_{1}^{(\phi)} = \bS_{1}^{(\phi)}(u_0^{\phi-1},y_0^{l-1})$ for $l \times l, l = 2^t$, kernel $K$ via LLRs $S_t^{(i)} =S_t^{(i)}(v_0^{i-1},y_0^{l-1})$, $i \geq \phi$ for   $F_t$. 

Namely, since $K$ and $F_t$ are invertible, we can write $TK = F_{t}$. Hence, any vector can be represented as 
$c_{0}^{l-1} = v_0^{l-1} F_{t} =u_{0}^{l-1}K$. It implies that $u_0^{l-1} = v_0^{l-1}T,$
or
\begin{equation}
\label{mInputTransitionExp}
u_\phi = \sum_{s = 0}^{l-1} v_s T[s,\phi] = \sum_{\substack{s = 0 \\T_{[s,\phi]} = 1}}^{\tau_\phi} v_s,
\end{equation}
where $\tau_\phi$ is the position of the last non-zero symbol in the $\phi$-th column of $T$. For simplicity we assume that all $\tau_{\phi}$ are distinct. The general case is considered in \cite{trofimiuk2020windowArXiv}.

The relations between input vectors $u$ and $v$ of polarizing transforms $K$ and $F_t$ can be used to compute LLRs for $K$ via LLRs for $F_t$. Let $h_\phi = \underset{0 \leq \phi' < \phi}{\max} \tau_{\phi'}$. Observe that it is possible to reconstruct $u_0^{\phi-1}$ from $v_0^{h_{\phi}-1}$ via \eqref{mInputTransitionExp}.  Computation of LLRs $S_t^{(h_\phi)}(v_0^{h_\phi-1},y_0^{l-1})$ \cite{trofimiuk2020windowArXiv} requires exact values of all elements of $v_0^{h_\phi-1}$. However, if  $h_\phi > \phi$, then some values of $v_0^{h_\phi-1}$ are independent from $u_0^{\phi-1}$ and, therefore, unknown. It means that one should consider vectors $v_0^{h_\phi-1}$ with all possible values of unknown bits and compute the corresponding LLRs $S_t^{(h_\phi)}$. 
 
 Let
$
\mathcal D_\phi = [h_\phi]\setminus  \{\tau_0,\tau_1,\dots,\tau_{\phi-1}\}
$
 be a \textit{decoding window} (DW), i.e. the set of indices of independent components of $v_0^{h_\phi-1}$, where 
 $|\mathcal D_\phi| = h_\phi - \phi$ \cite{trofimiuk2020windowArXiv}. It can be seen that \cite{trofimiuk2020windowArXiv}
\begin{align}
\bS_{1}^{(\phi)} = \max_{v_0^{h_{\phi}}\in\mathcal Z_{\phi}^{(0)}} R_y(v_0^{h_\phi}) -
\max_{v_0^{h_{\phi}}\in\mathcal Z_{\phi}^{(1)}} R_y(v_0^{h_\phi}),
\label{mKernLLR}
\end{align}
where $\mZ_\phi^{(b)}$ is the set of vectors $v_0^{h_\phi}$, where 
$v_s \in \bF_2, s\in \mD_\phi$, and the values of $v_t, t \in [h_\phi+1] \backslash \mathcal D_\phi,$ are obtained according to expression \eqref{mInputTransitionExp} under condition $u_\phi = b$.

The number of path scores to be computed  in \eqref{mKernLLR} is given by 
$|\mZ_{\phi}| = 2^{|\mZ_\phi^{(0)} \cup \mZ_\phi^{(1)}|+1}$. 
To obtain these path scores, one need compute $2^{|\mD_\phi|}$ LLRs $S_t^{(h_\phi)}(v_0^{h_\phi-1},y_0^{l-1})$. Equation \ref{mKernLLR} can be directly used for kernel processing, however, a lot of simplification for this algorithm was proposed in \cite{trofimiuk2020windowArXiv}.

In general, one has 
$\max_{i \in [l]}|\mathcal D_i| = O(l)$ for an arbitrary  $K$. There are some methods to construct polarization kernels, which admit  low complexity window processing \cite{trofimiuk2019construction32}, \cite{abbasi2020large}.

\subsection{Processing of shortened kernels}

Consider shortening of $l \times l, l = 2^t $ kernel $K$ on $s$ columns via pattern $\mP$, which resulted in kernel $K'$. It is convenient for further discussion to assume that kernel $K$ does not require addition of some rows $K[i]$ to rows $K[j]$ with $j < i$ during shortening. Actually, any kernel can be transformed to such form without changing of polarization properties. 

Let $\mR$ be a set of $s$ indices of rows of $K$ removed by shortening. Observe that $u_r = 0, r \in \mR$. The kernel $K'$ can be processed by WP\ algorithm for kernel $K$ by setting $y_p = \infty, p \in \mP,$ and skipping processing of phases $r \in \mR$. 

Observe that some elements of $v_0^{l-1}$ can also be set to zero. Namely, if expression $u_r = v_{\tau_r}$ occurs in \eqref{mInputTransitionExp}, thus $v_{\tau_r} = 0$. This also leads to excluding index $\tau_r$ from all DWs $\mD_\phi, \phi \in [l]$. Let $\mD_\phi' = \set{h|h \in \mD_\phi, v_h \ne 0}$.
Reduced DW $\mD_\phi'$ at phase $\phi$ results in reduced by 
$2^{|\mD_\phi| -|\mD_\phi'|}$ times number of LLRs $S_t^{(h_\phi)}$ required for computing \eqref{mKernLLR}, which greatly reduce overall processing complexity.

Recall that each LLR $S_t^{(h_\phi)}(v_0^{h_\phi-1},y_0^{l-1})$ for $v_0^{h_\phi-1} \in \mZ_\phi$ is computed recursively via expressions \eqref{mMinSum1}--\eqref{mMinSum2}. On each layer $\lambda \in [t+1]$ of this recursion intermediate LLRs $S_{\lambda}^{(j)} = S_{\lambda}^{(j)}(\bar v_0^{j-1},\bar y_0^{2^\lambda-1})$ are arising. After shortening the values $S_0^{0}(y_r) = \infty, r \in \mR,$ and, therefore, some $S_\lambda^{(j)} = \infty$. One does not need to compute  such $S_\lambda^{(j)}$.
  

